Knowledge Distillation Approaches for Accurate and Efficient Recommender System

Despite its breakthrough in classification problems, Knowledge distillation (KD) to recommendation models and ranking problems has not been studied well in the previous literature. This dissertation is devoted to developing knowledge distillation methods for recommender systems to fully improve the performance of a compact model. We propose novel distillation methods designed for recommender systems. The proposed methods are categorized according to their knowledge sources as follows: (1) Latent knowledge: we propose two methods that transfer latent knowledge of user/item representation. They effectively transfer knowledge of niche tastes with a balanced distillation strategy that prevents the KD process from being biased towards a small number of large preference groups. Also, we propose a new method that transfers user/item relations in the representation space. The proposed method selectively transfers essential relations considering the limited capacity of the compact model. (2) Ranking knowledge: we propose three methods that transfer ranking knowledge from the recommendation results. They formulate the KD process as a ranking matching problem and transfer the knowledge via a listwise learning strategy. Further, we present a new learning framework that compresses the ranking knowledge of heterogeneous recommendation models. The proposed framework is developed to ease the computational burdens of model ensemble which is a dominant solution for many recommendation applications. We validate the benefit of our proposed methods and frameworks through extensive experiments. To summarize, this dissertation sheds light on knowledge distillation approaches for a better accuracy-efficiency trade-off of the recommendation models.

==> chapters/ckd/sections/000Abstract.tex <==
Recent recommender systems have shown remarkable performance by using a large and sophisticated model. 
Further, an ensemble of heterogeneous models is known to achieve significantly increased accuracy over a single model.
However, it is exceedingly costly because it requires resources and inference latency proportional to the number of models, which remains the bottleneck for production.
Our work aims to transfer the ensemble knowledge of heterogeneous teachers to a lightweight student model using knowledge distillation (KD), to reduce the huge inference costs while retaining high accuracy.
Through an empirical study, we find that the efficacy of distillation severely drops when transferring knowledge from heterogeneous teachers.
Nevertheless, we show that an important signal to ease the difficulty can be obtained from the teacher training trajectory.
This paper proposes a new KD framework, named \proposed, that guides the student model by transferring easy-to-hard sequences of knowledge generated from the teachers' trajectories.
To provide guidance according to the student's learning state, \proposed uses \textit{dynamic knowledge construction} to provide progressively difficult ranking knowledge and \textit{adaptive knowledge transfer} to gradually transfer finer-grained ranking information.
Our comprehensive experiments show that \proposed significantly improves the distillation quality and the generalization of the student model.




==> chapters/ckd/sections/070Conclusion.tex <==
We propose a new HetComp framework to compress the ensemble knowledge of heterogeneous recommendation models into a lightweight model, so as to reduce the huge inference costs while retaining high accuracy.
From our analysis, we show that distillation from heterogeneous teachers is particularly challenging and teachers' training trajectories can help to ease such high learning difficulties.
Based on the idea of easy-to-hard learning, HetComp uses \textit{dynamic knowledge construction} to provide progressively difficult ranking knowledge and \textit{adaptive knowledge transfer} to gradually transfer finer-grained ranking information.
We provide extensive experiments showing that HetComp significantly improves the distillation quality and the generalization of the student model.
We leave attempts to further enhance the ensemble knowledge (e.g., trying more diverse model combinations) for future study.


==> chapters/concf/sections/060Conclusion.tex <==
We first provide in-depth analyses showing the necessity of consolidating knowledge from heterogeneous OCCF objectives, which has not been studied well in the previous studies.
Motivated by the analyses, we propose a novel ConCF framework whereby the multiple heads trained by heterogeneous objectives collaboratively evolve based on their complementarity throughout the training process.
ConCF generates the ranking consensus by selectively reflecting the reliable predictions from each head, and enhances the heads by using the consensus.
The improved heads generate more accurate consensus again, interactively boosting the recommendation quality.
We validate the superiority of ConCF by extensive experiments.
Especially, the comparison with various training schemes shows the effectiveness of each proposed component.
We leave the study of exploiting the complementarity from multiple factors (e.g., model size, initialization) simultaneously for future work.


% \vspace{0.1cm}
% \noindent
% \textbf{Acknowledgement.}
% This work was supported by the IITP grant funded by the MSIT (No.2018-0-00584, No.2019-0-01906), the NRF grant funded by the MSIT (No.2020R1A2B5B03097210), the Technology Innovation Program funded by the MOTIE (No.20014926), 
% and a grant of the Korea Health Technology R\&D Project through the KHIDI, funded by the MOHW (HI18C2383).

==> chapters/derrd/sections/expert_selection_map.tex <==
\begin{figure}[t]
\vspace{-0.1cm}
\begin{subfigure}[t]{0.5\linewidth}
    \includegraphics[width=\linewidth]{chapters/derrd/images/balance legend2.png}
\end{subfigure} 
\\
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\linewidth]{chapters/derrd/images/balance_attention.png}
    \caption*{Attention}
\end{subfigure} 
\hspace*{-0.07in}
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\linewidth]{chapters/derrd/images/balance_one_big.png}
    \caption*{One expert (large)}
\end{subfigure}
\hspace*{-0.07in}
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\linewidth]{chapters/derrd/images/balance_selection.png}
    \caption*{DE (selection)}
\end{subfigure} 
\caption{Performance (N@20) gain map (BPR with $\phi=0.1$ on Foursquare).}
\label{fig:pgain}
\end{figure}
\begin{figure}[t]
\vspace*{-0.2cm}
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\linewidth]{chapters/derrd/images/selection0.png}
    \caption{Epoch 0}
\end{subfigure} 
\hspace*{-0.07in}
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\linewidth]{chapters/derrd/images/selection10.png}
    \caption{Epoch 20}
\end{subfigure}
\hspace*{-0.07in}
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[width=\linewidth]{chapters/derrd/images/selection15.png}
    \caption{Train Done}
\end{subfigure} 
\caption{Expert selection map of DE. Each color corresponds to an expert (BPR with $\phi=0.1$ on Foursquare).}
\label{fig:de-rrd_selection_map}
\end{figure}



==> chapters/irrrd/sections/main_result1_f.tex <==
\begin{table}[ht]
\setlength\tabcolsep{3.5pt}
\footnotesize
%\renewcommand{\arraystretch}{0.65}
% \setlength\tabcolsep{5.5pt}
%\small
%\RowStretch{0.2}
%\renewcommand{\arraystretch}{0.4}
  \caption{Recommendation performances of BPR ($\phi=0.1$). *** and **** indicate $p \leq 0.0005$, and $p \leq 0.00005$ for the paired t-test of IR-RRD vs. the best baseline on H@5.}
  
  \begin{tabular}{clccc ccc ccc}
    \toprule 
     Dataset & KD Method & H@5 & M@5 & N@5 & H@10 & M@10 & N@10 & H@20 & M@20 & N@20 \\
    \midrule
    &MOSTPOP&0.1389&0.0820&0.0960&0.1920&0.0890&0.1131&0.2610&0.0938&0.1305\\
    \cmidrule{2-11}
     &Teacher&0.1016&0.0574&0.0682&0.1470&0.0633&0.0828&0.2073&0.0673&0.0978\\
     \multirow{3}{*}{\rotatebox{90}{CiteULike}}&Student&0.0630&0.0348&0.0417&0.0973&0.0396&0.0534&0.1460&0.0428&0.0652\\
     &RRD&0.0730&0.0410&0.0489&0.1109&0.0460&0.0611&0.1670&0.0498&0.0752\\
     \cmidrule{2-11}
     &IR-RRD ****&\textbf{0.0854}&\textbf{0.0478}&\textbf{0.0571}&\textbf{0.1266}&\textbf{0.0532}&\textbf{0.0704}&\textbf{0.1832}&\textbf{0.0571}&\textbf{0.0846}\\
    \midrule
    &MOSTPOP&0.1370&0.0909&0.1023&0.1811&0.0967&0.1165&0.2390&0.1007&0.1312\\
    \cmidrule{2-11}
    &Teacher&0.0809&0.0488&0.0566&0.1137&0.0532&0.0670&0.1615&0.0564&0.0789\\
    \multirow{3}{*}{\rotatebox{90}{Foursquare}}&Student&0.0645&0.0388&0.0454&0.0911&0.0425&0.0544&0.1333&0.0453&0.0648\\
    &RRD&0.0711&0.0426&0.0498&0.1015&0.0466&0.0594&0.1464&0.0496&0.0708\\
    \cmidrule{2-11}
    &IR-RRD ***&\textbf{0.0761}&\textbf{0.0466}&\textbf{0.0539}&\textbf{0.1086}&\textbf{0.0507}&\textbf{0.0640}&\textbf{0.1557}&\textbf{0.0537}&\textbf{0.0749}\\
%    \cmidrule{2-11}
%     &\textit{Improv.b}&3.76\%&3.64\%&3.69\%&2.33\%&3.25\%&2.94\%&1.11\%&3.11\%&2.33\%\\
%    &\textit{Improv.s}&9.37\%&11.33\%&10.62\%&5.83\%&10.13\%&8.57\%&2.62\%&9.35\%&6.65\%\\
    \bottomrule
  \end{tabular}
  \label{tab:IRRRD_main_BPR}
\end{table}    


==> chapters/irrrd/sections/main_result2_f.tex <==

\begin{table}[ht]
\setlength\tabcolsep{3.5pt}
\footnotesize
%\renewcommand{\arraystretch}{0.65}
%\small
%\RowStretch{0.2}
%\renewcommand{\arraystretch}{0.4}
  \caption{Recommendation performances of NeuMF ($\phi=0.1$). 
  * and ** indicate $p \leq 0.05$, $p \leq 0.005$ for the paired t-test of IR-RRD vs. the best baseline on H@5.}
  
  \begin{tabular}{clccc ccc ccc}
    \toprule 
     Dataset & KD Method & H@5 & M@5 & N@5 & H@10 & M@10 & N@10 & H@20 & M@20 & N@20 \\
    \midrule
    &MOSTPOP&0.1389&0.0820&0.0960&0.1920&0.0890&0.1131&0.2610&0.0938&0.1305\\
    \cmidrule{2-11}
    &Teacher&0.0985&0.0584&0.0682&0.1420&0.0640&0.0818&0.2010&0.0677&0.0955\\
    \multirow{3}{*}{\rotatebox{90}{CiteULike}}&Student&0.0537&0.0275&0.034&0.0839&0.0319&0.0446&0.1219&0.0349&0.0549\\
    &RRD &0.0660&0.0329&0.0410&0.1078&0.0384&0.0544&0.1696&0.0426&0.0701\\
    \cmidrule{2-11}
    &IR-RRD **&\textbf{0.0704}&\textbf{0.0380}&\textbf{0.0458}&\textbf{0.1170}&\textbf{0.0438}&\textbf{0.0601}&\textbf{0.1838}&\textbf{0.0480}&\textbf{0.0762}\\
    \midrule
    &MOSTPOP&0.1370&0.0909&0.1023&0.1811&0.0967&0.1165&0.2390&0.1007&0.1312\\
    \cmidrule{2-11}
    &Teacher&0.0704&0.0406&0.0479&0.1065&0.0453&0.0595&0.1541&0.0485&0.0714\\
    \multirow{3}{*}{\rotatebox{90}{Foursquare}}&Student&0.0436&0.0225&0.0277&0.0716&0.0262&0.0367&0.1151&0.0291&0.0476\\
    &RRD &0.0568&0.0307&0.0371&0.0894&0.0351&0.0477&0.1365&0.0382&0.0595\\
    \cmidrule{2-11}
    &IR-RRD *&\textbf{0.0589}&\textbf{0.0318}&\textbf{0.0385}&\textbf{0.0902}&\textbf{0.0360}&\textbf{0.0485}&\textbf{0.1403}&\textbf{0.0391}&\textbf{0.0605}\\
    \bottomrule
  \end{tabular}
  \label{tab:IRRRD_main_NeuMF}
\end{table}


==> chapters/irrrd/sections/model_size_figure1_f.tex <==

%%% K-grpah
\begin{figure}[h!]
\centering
\begin{subfigure}[t]{0.50\linewidth}
% \centering
% \begin{centering}
    \includegraphics[width=\linewidth]{chapters/irrrd/images/legend_f.png}
% \end{centering}
\end{subfigure}

\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{chapters/irrrd/images/BPR_C_H.png}
%    \caption{H@5 (Base Model: BPR)}
\end{subfigure}
\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{chapters/irrrd/images/BPR_4_H.png}
%    \caption{N@5 (Base Model: BPR)}
\end{subfigure} 
\\
\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{chapters/irrrd/images/BPR_C_N.png}
%    \caption{H@5 (Base Model: NeuMF)}
\end{subfigure} 
\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{chapters/irrrd/images/BPR_4_N.png}
%    \caption{H@5 (Base Model: BPR)}
\end{subfigure}
% \\
% \begin{subfigure}[t]{0.48\linewidth}
%     \includegraphics[width=\linewidth]{figs/B_C_m5.png}
% %    \caption{N@5 (Base Model: BPR)}
% \end{subfigure} 
% \begin{subfigure}[t]{0.48\linewidth}
%     \includegraphics[width=\linewidth]{figs/B_4_m5.png}
% %    \caption{H@5 (Base Model: NeuMF)}
% \end{subfigure} 
%\caption*{(a) CiteULike}
% \caption{Recommendation Performance on CiteULike dataset across three different model sizes. (Red dotted line: Teacher)}
%\caption*{(b) Foursqure}
\centering
\label{fig:IRRRD_model_size_BPR}
\caption{Recommendation Performance of BPR across three different student model sizes. (Red dotted line: Teacher)}
\end{figure}


==> chapters/irrrd/sections/model_size_figure2_f.tex <==

%%% K-grpah
\begin{figure}[h!]
\centering
\begin{subfigure}[t]{0.50\linewidth}
% \centering
% \begin{centering}
    \includegraphics[width=\linewidth]{chapters/irrrd/images/legend_f.png}
% \end{centering}
\end{subfigure}

\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{chapters/irrrd/images/N_C_H.png}
%    \caption{H@5 (Base Model: BPR)}
\end{subfigure}
\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{chapters/irrrd/images/N_4_H.png}
%    \caption{N@5 (Base Model: BPR)}
\end{subfigure} 
\\
\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{chapters/irrrd/images/N_C_N.png}
%    \caption{H@5 (Base Model: NeuMF)}
\end{subfigure} 
\begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{chapters/irrrd/images/N_4_N.png}
%    \caption{H@5 (Base Model: BPR)}
\end{subfigure}
% \\
% \begin{subfigure}[t]{0.48\linewidth}
%     \includegraphics[width=\linewidth]{figs/B_C_m5.png}
% %    \caption{N@5 (Base Model: BPR)}
% \end{subfigure} 
% \begin{subfigure}[t]{0.48\linewidth}
%     \includegraphics[width=\linewidth]{figs/B_4_m5.png}
% %    \caption{H@5 (Base Model: NeuMF)}
% \end{subfigure} 
%\caption*{(a) CiteULike}
% \caption{Recommendation Performance on CiteULike dataset across three different model sizes. (Red dotted line: Teacher)}
%\caption*{(b) Foursqure}
\centering
\label{fig:IRRRD_model_size_BPR}
\caption{Recommendation Performance of BPR across three different student model sizes. (Red dotted line: Teacher)}
\end{figure}


==> chapters/sscdr/main.tex <==
% terminologies
\newcommand{\rs}{RS\xspace}
\newcommand{\cdr}{CDR\xspace}
\newcommand{\cf}{CF\xspace}
\newcommand{\mf}{MF\xspace}
\newcommand{\pmf}{PMF\xspace}

% methods
\newcommand{\proposed}{SSCDR\xspace}
\newcommand{\proposednoinf}{SSCDR\textsubscript{naive}\xspace}
\newcommand{\proposedinf}{SSCDR\xspace}
\newcommand{\emcdr}{EMCDR\xspace}
\newcommand{\emcdrbpr}{EMCDR-BPR\xspace}
\newcommand{\emcdrcml}{EMCDR-CML\xspace}
\newcommand{\bpr}{BPR\xspace}
\newcommand{\cml}{CML\xspace}
\newcommand{\cbmf}{CBMF\xspace}
\newcommand{\itempop}{ITEMPOP\xspace}

% notations
\newcommand{\srcdomain}{$\mathcal{D}^s$\xspace}
\newcommand{\tgtdomain}{$\mathcal{D}^t$\xspace}
\newcommand{\overlappinguser}{$\mathcal{O U}$\xspace}
\newcommand{\Rone}{R_\text{oou}\xspace}
\newcommand{\Rtwo}{R_\text{oos}\xspace}
\newcommand{\neighborofuseri}{\small$\mathcal{N I}^s_i$\normalsize\xspace}
\newcommand{\neighborofitemj}{\small$\mathcal{N U}^s_j$\normalsize\xspace}


\input{chapters/sscdr/sections/000abstract}


\section{Introduction}
\input{chapters/sscdr/sections/010introduction}

\section{Preliminaries}
\label{sec:preliminary_sscdr}
\input{chapters/sscdr/sections/020preliminaries}



\input{chapters/sscdr/sections/030analysis}


% 
\section{Proposed Method---SSCDR}
\input{chapters/sscdr/sections/040method}

\section{Experiments}
\input{chapters/sscdr/sections/050experiments}


\section{Related Work}
\input{chapters/sscdr/sections/060related}

\section{Summary}
\input{chapters/sscdr/sections/070conclusion}



==> chapters/sscdr/sections/000abstract.tex <==

%Recently, cross-domain recommendation (\cdr) has gained much attention because it alleviates the data sparsity problem of single-domain recommendation by integrating the information about users' preferences on items from multiple domains.
%In this work, we focus on recommending cross-domain items to the users who have not interacted with those items at all (i.e., potential users, so-called \textit{cold-start users}).

Providing accurate recommendations to newly joined users (or potential users, so-called \textit{cold-start users}) has remained a challenging yet important problem in recommender systems. 
To infer the preferences of such cold-start users based on their preferences observed in other domains, several cross-domain recommendation (CDR) methods have been studied.
The state-of-the-art Embedding and Mapping approach for \cdr (\emcdr) aims to infer the latent vectors of cold-start users by supervised mapping from the latent space of another domain.
In this paper, we propose a novel \cdr framework based on semi-supervised mapping, called \proposed, which effectively learns the cross-domain relationship even in the case that only a few number of labeled data is available.
To this end, it first learns the latent vectors of users and items for each domain so that their interactions are represented by the distances, then trains a cross-domain mapping function to encode such distance information by exploiting both overlapping users as labeled data and all the items as unlabeled data.
In addition, \proposed adopts an effective inference technique that predicts the latent vectors of cold-start users by aggregating their neighborhood information.
Our extensive experiments on different \cdr scenarios show that \proposed outperforms the state-of-the-art methods in terms of \cdr accuracy, particularly in the realistic settings that a small portion of users overlap between two domains.

==> chapters/sscdr/sections/010introduction.tex <==

% CDR 설명
As an increasing number of users interact with one or more their interest domains, recent recommender systems (\rs) started to leverage user-item interactions (e.g., ratings or feedbacks) collected from multiple domains to improve the quality of recommendations, so-called cross-domain recommendation (\cdr)~\cite{EMCDR2017,CBMF2015,hu2018mtnet,bayesian2018,autoencoder_CDR_2019_AAAI,conet2018,CDRimprove2018}.
\cdr aims to transfer the knowledge acquired from a domain to another domain, and this inter-domain information exchange is quite helpful to combat the data sparsity problem, which is one of the long-standing problems in conventional \rs.

% cold-start user problem 중요성 / challenge 설명
Most \cdr methods~\cite{CDRimprove2018,conet2018,dcdcsr2018,CDRforsparsityreduction} are mainly interested in improving the overall recommendation accuracy for a target domain by the help of the users who also exist in other domains (i.e., \textit{overlapping users}). Thus, they cannot make recommendations to the users who are newly joined or have not interacted with any items yet (i.e., \textit{cold-start users}).
%addressing the data sparsity problem~\cite{dcdcsr2018, conet2018, CDRimprove2018, CDRforsparsityreduction}, so they have focused on only .
This is another important task in \cdr, and it is more technically challenging as well as has great values from a practical perspective~\cite{CBMF2015}.
%For example, providers want to cross-sell a wide variety of items to a large number of newly joined users, 
To this end, \rs should be able to infer the preferences of such cold-start users based on their preferences observed in other domains.
For example, providers can recommend video-domain items to the users who want to try videos for the first time by analyzing their preferences in a book-domain.
In this paper, we use the term ``target-domain'' for the domain that we try to recommend, and ``source-domain'' for the domain that we transfer the knowledge of cold-start users' preferences from.

% EMCDR 어프로치 설명
To tackle this challenge, several recent work~\cite{EMCDR2017, autoencoder_CDR_2019_AAAI} focus on the Embedding and Mapping approach (\emcdr) which matches two latent spaces, where users' preferences on items are encoded respectively for a source-domain and a target-domain, by using the overlapping users of the two domains as anchor points.
It trains a mapping function from the source-domain into the target-domain in a supervised manner so that it minimizes the distance between the actual latent vector in the target-domain and the approximated latent vector transferred from the source-domain for each overlapping user.
After inferring the latent vectors of cold-start users by the trained mapping function, \emcdr is able to provide recommendations to the cold-start users.

% 기존 방법의 한계점
% However, the \emcdr~\cite{} approach is not practical enough as they learns the cross-domain relationship only by supervised manner, which makes the methods largely dependent on the number of the overlapping users.
However, existing EMCDR-based methods \cite{EMCDR2017,dcdcsr2018, autoencoder_CDR_2019_AAAI} have a limited performance in real-world \cdr scenarios for the following reasons.
1) The \emcdr approach is only based on a supervised loss, which makes the mapping function biased to a small number of the overlapping users who are used as the anchors for training. 
From our in-depth analysis on the Amazon dataset, we found that the average ratio of the overlapping users to total users of any two domains is less than 5\%. However, all the methods were evaluated in the experimental settings where a lot of users (up to 90\%) are overlapped~\cite{bayesian2018, EMCDR2017,autoencoder_CDR_2019_AAAI, hu2018mtnet}, which distorts the real-world distribution.
2) They basically model the user-item interaction as the \textit{inner-product} of their latent vectors, which makes a latent space violate triangle inequality~\cite{triangle_inequality_2012};
in such spaces, the similarities among users and among items are not correctly captured~\cite{CML,PME2018}.
It eventually degrades the performance of collaborative filtering for each domain and also that of the cross-domain mapping because their mapping function is optimized by the \textit{distance}-based supervised loss.
% They basically model the user-item interaction as the inner-product of their latent vectors, which is inconsistent with the supervised loss (i.e., l2 distance) used to train the cross-domain mapping function.
% 
\begin{comment}
They basically model the user-item interaction as the inner-product of their latent vectors. 
This modeling inherently has limitations that the inner-product makes a latent space violate \textit{triangle inequality} and inconsistency between cross-domain mapping optimized by the supervised loss (i.e.,l2 distance) and the user-item interaction optimized by the inner-product;
in such spaces, the l2 distance among users and among items do not correctly represent their similarities~\cite{CML,PME2018}.
It eventually degrades the cross-domain recommendation accuracy.
\end{comment}

%(This will be further discussed in Section~\ref{sec:analysis}.)
%2) Some of the methods require side information such as users' demographic information~\cite{bayesian2018} and review texts on items~\cite{autoencoder_CDR_2019_AAAI, hu2018mtnet} to infer the latent vectors of cold-start users from content-based similarities, but these auxiliary data sources are neither always available nor informative enough to learn the users' preference on items~\cite{nguyen2017hierarchical}.

% 우리 메서드 소개, 장점 어필
In this paper, we propose a Semi-Supervised framework for Cross-Domain Recommendation to cold-start users (\proposed) that works well even in the case that there are only a few overlapping users in both the domains.
To effectively capture the cross-domain relationship, \proposed first learns the latent vectors of users and items in \textit{metric spaces} to capture user-user similarities as well as user-item interactions in their distances.
Then, it trains a cross-domain mapping function based on a \textit{semi-supervised approach}, which optimizes the function to approximate the ground-truths of overlapping users (\textit{labeled data}), and to encode their interactions with items simultaneously (\textit{unlabeled data}).
In addition, we develop a novel technique to accurately infer the latent vectors of the cold-start users considering the neighborhood of the users.

Our extensive experiments demonstrate that \proposed outperforms all other baselines in terms of both the recommendation accuracy and the quality of cross-domain latent vector mapping. 
\proposed shows the best \cdr accuracy for cold-start users even in case that the number of overlapping users is very small, which follows a realistic data distribution, whereas the performances of the other methods drastically drop.
Furthermore, we quantitatively validate that \proposed is capable of inferring the latent vectors of cold-start users more accurately than the other methods, and qualitatively compare the target latent spaces induced by \proposed and the others.

\begin{comment}
The main contributions of this paper are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item Through our exhaustive analyses on real-world \cdr scenarios, we point out that only a small portion of users overlaps between two domains. Based on the results, we also criticize that most existing \cdr methods have been validated in the experimental settings that are distant from reality.
    \item We propose a general framework to recommend target-domain items to cold-start users based on a semi-supervised approach, which makes the cross-domain mapping function generalize much better than supervised one. It also adopts the multi-hop neighborhood inference technique to best predict the latent vectors of cold-start users.
    \item We demonstrate the superiority of our framework by extensive experiments on 12 different settings. It achieves the best accuracy even with a limited number of overlapping users, and our qualitative analyses show that the semi-supervised approach and the inference technique are helpful to accurately infer the latent vectors of cold-start users. 
\end{itemize}
\end{comment}

==> chapters/sscdr/sections/020preliminaries.tex <==
We first formally describe the notations and our problem (Section~\ref{subsec:notation}), then review an embedding and mapping approach which is a conventional strategy for cross-domain recommendation (\cdr) (Section~\ref{subsec:emcdr}). 


\subsection{Notations and Problem Formulation}
\label{subsec:notation}
Suppose that we have two domains: a source-domain and a target-domain.
In this paper, we use the term ``target-domain'' for the domain that we try to recommend, and ``source-domain'' for the domain that we transfer the knowledge of users' preferences from.
We use the \cdr scenario that ``Book'' is the source-domain and ``Video'' is the target-domain as an example case.
Let $\mathcal { U }^s$, $\mathcal { U }^t$, $\mathcal { I }^s$, and $\mathcal { I }^t$ be the set of users and items in the source-domain and the target-domain, respectively. 
In most real-world cases, $ \mathcal { U } ^ s$ and $ \mathcal { U } ^ t $ are partially overlapped: the users who watch videos and also purchase books are a part of the total users. 
Thus, we define the set of overlapping users between the two domains by \overlappinguser$= \mathcal { U } ^ s \cap \mathcal { U } ^ t $.
In contrast, $\mathcal { I }^s$ and $\mathcal { I }^t$ are disjoint sets, so there is no item that both the domains have in common.
Given collaborative filtering (CF) information (i.e., implicit interactions between users and items) for each domain, we build a binary matrix that represents user-item interactions.
The binary matrix $\boldsymbol { R }^s \in \{0,1\}^{| \mathcal { U }^s | \times | \mathcal { I }^s |}$ includes user-book purchase interactions, and similarly, $\boldsymbol { R }^t \in \{0,1\}^{| \mathcal { U }^t | \times | \mathcal { I }^t |}$ includes user-video watching interactions.
%where each entry $r_{i,j}$ is 1 if a user $i$ has purchased a book $j$ and 0 otherwise. 
% where each entry $r_{i,k}$ is 1 if a user $i$ has watched a video $k$ and 0 otherwise.
We additionally use the notations \neighborofuseri for the set of the items that the user $i$ has interacted with in the source-domain (i.e., the neighbor items of the user $i$), and \neighborofitemj for the set of the users that previously interacted with the item $j$ in the source-domain (i.e., the neighbor users of the item $j$).
Our goal is to recommend top-$N$ items in $\mathcal { I }^t$ to \textit{cold-start users} who have not interacted with $\mathcal { I }^t$ at all.
In other words, we aim to recommend videos to users who have never watched videos but only purchased books.

\subsection{Embedding and Mapping Approach}
\label{subsec:emcdr}
The Embedding and Mapping approach for Cross-Domain Recommendation (\emcdr), which is a general \cdr strategy for cold-start users, is firstly proposed in~\cite{EMCDR2017}, and several methods have been proposed based on this approach~\cite{dcdcsr2018, autoencoder_CDR_2019_AAAI}.
\emcdr consists of 1) the embedding step for modeling users and items in latent spaces, and 2) the mapping step for learning the inter-domain relationship.

In the embedding step, \emcdr learns the user and item latent vectors for each domain by using Matrix Factorization (MF).
MF models the user-item interaction as the inner product of their latent vectors~\cite{koren2009matrix}.
Given a dataset that contains implicit interactions between users and items, the latent vectors are optimized based on the assumption that a user prefers interacted items to non-interacted items~\cite{BPR}. 
This can be formalized as the following pairwise loss:
\begin{equation*}
    \min _ { \mathbf { u } * , \mathbf { v } * } \sum _ { i \in \mathcal{U} } \sum _ { j \in \mathcal{NI}^{\,}_i } \sum _ { k \notin \mathcal{NI}^{\,}_i } - \log \sigma ( \mathbf { u } _ { i } ^ { \top } \mathbf { v } _ { j } - \mathbf { u } _ { i } ^ { \top } \mathbf { v } _ { k } ),
\end{equation*}
% regularizer 필요한가? -> 없어도 될 듯
where $\sigma$ is the sigmoid function, $\mathbf { u }_* \in \mathbb{R}^d$, $\mathbf { v }_* \in \mathbb{R}^d$ are user and item latent vectors, and $d$ is the dimension size of the latent vectors.
In this way, \emcdr learns the latent matrices $\boldsymbol { U }^s \in \mathbb { R }^{| \mathcal { U }^s | \times d}, \boldsymbol { V }^s \in \mathbb { R }^{| \mathcal { I }^s | \times d}$ from $\boldsymbol { R }^s$, and $\boldsymbol { U }^t \in \mathbb { R }^{| \mathcal { U }^t | \times d}, \boldsymbol { V }^t \in \mathbb { R }^{| \mathcal { I }^t| \times d}$ from $\boldsymbol { R }^t$.

In the mapping step, \emcdr learns a mapping function $f_\theta$ to capture the inter-domain relationship by utilizing the overlapping users as a bridge. 
The learning procedure is formalized as a supervised regression problem,
\begin{equation*}
    \min _ { \theta } \sum _ { i \in \mathcal{O U} } || f_{\theta} \left( \mathbf { u }^s_{ i }\right) - \mathbf { u }^t _ { i } ||^2.
\end{equation*}
%where $f$ is the Multi-Layer Perceptron (MLP) mapping function.
The mapping function is optimized to minimize the distance between the user latent vectors transferred from the source-domain by cross-domain mapping and the corresponding user latent vectors in the target-domain.
After training the mapping function, \emcdr can infer the target-domain latent vector of a cold-start user $i$ by
%and provide recommendations to them.
%For example, given a cold-start user $i$, \emcdr infers its latent vector as follows:
$\hat { \mathbf { u }}^t  _ { i }  = f_ { \theta } ( \mathbf { u }^s _ {i })$.
Using the inferred latent vector and the target-domain item vectors $\boldsymbol { V }^t$, \emcdr provides recommendations to the user.

The existing \emcdr-based methods have a limited performance for the following reasons.
First, the training of the mapping function only uses the supervised loss, whose performance is sensitive to the number of overlapping users.
%However, the mapping function trained by the supervised loss can successfully capture the complex relationship between two domains only if there are enough overlapping users to cover all over the latent spaces.
In particular, in case that there are a small number of the overlapping users, the mapping function is severely biased to them and fails to be generalized to the cold-start users.
Second, they learn the user-item interaction as the inner product of their latent vectors, which makes the latent space violate \textit{triangle inequality}~\cite{triangle_inequality_2012}.
As pointed out in~\cite{CML, PME2018}, the user-user and item-item similarities are not accurately modeled in such space. 
In addition, the supervised loss for the mapping function defined by the Euclidean distance is not fully compatible with their latent space, because the user-item interactions are captured in the space as the inner product, not the distance. 
%As a result, these limitations eventually degrade the performance of the cross-domain mapping function.





==> chapters/sscdr/sections/030analysis.tex <==
\label{sec:analysis}
In this section, based on our detailed analyses on the Amazon dataset\footnote{https://registry.opendata.aws/amazon-reviews/}, we clarify the challenge of the \cdr task and the limitation of existing \cdr methods.
The Amazon dataset is the largest public \cdr dataset, which contains more than 1.3 million users and 42 item domains.

First, we analyze two factors that have a significant impact on the \cdr performance for all possible cross-domain scenarios, determined by any two domains.
\begin{equation*}
\Rone = \frac{|\mathcal{O U}|}{|\mathcal { U } ^ s  \cup \mathcal { U } ^ t|}, \quad 
 \Rtwo = \frac{|\mathcal{O U}|}{|\mathcal { U } ^ s|}
\end{equation*}
The first factor is the ratio of the overlapping users over the union of the source-domain and the target-domain users, denoted by $\Rone$.
As \cdr methods usually use the overlapping users as a bridge to transfer knowledge between two domains, the overall performances could be improved as $\Rone$ increases.
The second factor is the ratio of the overlapping users over the source-domain users, denoted by $\Rtwo$. 
The higher $\Rtwo$, the more information of the source-domain can be used to learn the cross-domain relationship, which results in more accurate transfer of users in the source-domain.
Figure~\ref{fig:analysis} shows the histogram of $\Rone$ and $\Rtwo$.
We observe that cross-domain scenarios with $\Rone$ less than 10$\%$ account for 92$\%$ of the total scenarios.
Similarly, the scenarios with $\Rtwo$ less than 20$\%$ account for 83$\%$ of the total scenarios.

\begin{figure}[t]
\centering
\begin{minipage}[t]{0.498\linewidth}
    \includegraphics[height=4cm]{chapters/sscdr/images/total_percentage.png}
\end{minipage}%
    \hfill%
\begin{minipage}[t]{0.498\linewidth}
    \includegraphics[height=4cm]{chapters/sscdr/images/src_percentage.png}
\end{minipage} 
\caption{Histograms of $\Rone$ and $\Rtwo$ on cross-domain scenarios (Red dotted lines: the averages)}
\label{fig:analysis}
\end{figure}

We also compare the experimental settings used in the recent \cdr methods for cold-start users, including our proposed method.
In~Table~\ref{tab:othermethod}, all the previous work have evaluated their methods in the experimental settings where both $\Rone$ and $\Rtwo$ range from 20$\%$ to 90$\%$.
Most of them first start from the case that all users are \textit{completely overlapped} between the two domains and gradually remove the users in the target-domain. 
However, as shown in Figure~\ref{fig:analysis}, scenarios with $\Rone$ larger than 20$\%$ rarely exist, and scenarios with $\Rtwo$ larger than 20$\%$ only account for 19$\%$ of the total scenarios.
Although our data analyses do not cover all real-world \cdr scenarios, at least we confirm that the existing methods have proved their effectiveness in the experimental environments that are distant from reality.

\begin{table}[t]
\centering
% \setlength\tabcolsep{3pt}
% \renewcommand{\arraystretch}{0.95}
  \caption{Experimental settings (training set) of recent CDR methods for cold-start users and SSCDR }
  \label{tab:othermethod}
  \begin{tabular}{cccc}
    \toprule
    Methods& $\Rone$ & $\Rtwo$  & Side Information\\
    \midrule
    GCBAN \cite{bayesian2018} & 20 $\sim$ 80\% & 20 $\sim$ 80\% & Yes\\
    RC-DFM \cite{autoencoder_CDR_2019_AAAI} & 20 $\sim$ 80\% & 20 $\sim$ 80\% & Yes\\ 
    EMCDR \cite{EMCDR2017} & 50 $\sim$ 90\% & 50 $\sim$ 90\% & No\\
    SSCDR  & 0.2 $\sim$ 5.6\% & 0.3 $\sim$ 21.2\% & No\\
    \bottomrule
\end{tabular}
\end{table}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{chapters/sscdr/images/method.png}
  \caption{Illustration of the proposed semi-supervised mapping approach.
(a) Learned metric space for the source-domain (solid lines: observed user-item interactions).
(b) Transferred locations are confined to the overlapping user 1.
(c) The supervised loss in Eq.~\eqref{eq:suploss} creates a gradient that pulls the transferred user 1 to the user 1. The unsupervised loss in Eq.~\eqref{eq:unsuploss} creates a gradient that pulls positive item 1 closer to the user 1 and pushes negative item 2.
(d) Transferred locations of user 1, item 1 and item 2 are adjusted. As a result, transferred locations of user 2 and user 3 are naturally adjusted.
}
  \label{fig:method}
\end{figure}













==> chapters/sscdr/sections/040method.tex <==
In this section, we provide the details of \proposed framework which bridges semi-supervised learning to \cdr. 
%With the help of a semi-supervised approach, \proposed is able to effectively learn cross-domain relationship even with only a small number of overlapping users. 
%\proposed learns latent vectors of users and items in a metric space where user-item similarities (or relations) are captured as their distances, and it infers the latent vectors of cold-start users based on such similarity information.
Our proposed framework consists of the following three major steps. 
In the first step, \proposed learns user and item latent vectors in metric spaces for the source-domain and target-domain, respectively (Section~\ref{subsec:modeling}). 
In the second step, \proposed trains a mapping function that captures the cross-domain relationships between the two metric spaces (Section~\ref{subsec:mapping}).
In the third step, \proposed infers the latent vectors of cold-start users based on their neighborhood in the source-domain, then recommends the target-domain items to cold-start users (Section~\ref{subsec:inference}).
Algorithm~\ref{alg:framework} describes the overall process of our framework.

% 각 도메인 별, Notation 정의 다시해야하나?
\subsection{Collaborative Filtering in Metric Space}
\label{subsec:modeling}
The first step of the \proposed framework is to learn a metric space for each domain.
To be specific, we embed users and items into the low-dimensional metric space where a user's preference on an item is inversely proportional to their Euclidean distance.
The distance between a user $i$ and an item $j$ is defined as
\begin{equation}
    \begin{aligned}
    d(\mathbf{u}_i,\mathbf{v}_j) = \left\| \mathbf { u }_i - \mathbf { v }_j \right\|^ 2.
    \end{aligned}
\end{equation}
We optimize the space so that the distance between a user and its interacted items becomes smaller than the distance between the user and its non-interacted items. 
This collaborative filtering in metric space~\cite{CML} is formulated by the following loss function:
\begin{equation}
\begin{aligned}
\label{eq:CMLLoss}
    \mathcal {L} &=  \sum _ { i \in \mathcal{U} } \sum _ { j \in \mathcal{NI}^{\,}_i } \sum _ { k \notin \mathcal{NI}^{\,}_i } \left[ m + d \left(\mathbf { u }_ {i},  \mathbf { v }_ { j } \right) - d \left( \mathbf { u }_ { i } , \mathbf { v }_ { k } \right) \right]_{ +, }\\
        & \hspace{15mm} s.t.\hspace{3mm}||\mathbf{u}_{*}||^{2} \leq 1 \text{ and } ||\mathbf{v}_{*}||^{2} \leq 1, 
\end{aligned}
\end{equation}
where $m$ is margin size and $[x]_{+} = \max(x,0)$ is the standard hinge loss. 
We also add the unit sphere constraint to prevent user and item vectors from spreading too widely. 
This constraint is enforced by normalizing latent vectors (i.e., $\mathbf { u }_{*}\leftarrow \mathbf { u }_{*}/\text{max}(1,\left\|\mathbf { u }_{*}\right\|_2),\hspace{1mm}\mathbf { v }_{*}\leftarrow \mathbf { v }_{*}/\text{max}(1,\left\|\mathbf { v }_{*}\right\|_{2}) $, as done in~\cite{CML}. 


\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

\begin{algorithm}[t]
\small
\SetAlgoLined
\nonl \textbf{Require:} The interaction matrices, user and item sets of each domain $\boldsymbol{R}^s$,  $\boldsymbol{R}^t$, $\mathcal{U}^s$, $\mathcal{U}^t$, $\mathcal{V}^s$, and $\mathcal{V}^t$\\
\nonl \textbf{Ensure:} Recommend top-$N$ target-domain items to cold-start users\\

\vspace{2pt} \nonl \textbf{(1) Collaborative Filtering in Metric Space}\\
Learn \{$\boldsymbol { U }^s$, $\boldsymbol { V }^s$\} from $\boldsymbol{R}^s$ in a metric space\\
Learn \{$\boldsymbol { U }^t$, $\boldsymbol { V }^t$\} from $\boldsymbol{R}^t$ in a metric space\\

\vspace{2pt} \nonl \textbf{(2) Semi-Supervised Metric Space Mapping}\\
Learn the mapping function $f_\theta(\cdot)$ between two metric spaces\\

\vspace{2pt} \nonl \textbf{(3) Multi-hop Neighborhood Inference}\\
Compute neighborhood-aggregated user latent vectors \footnotesize$\boldsymbol{U}^{s,H}$\small\\
Infer the latent vectors of cold-start users \footnotesize$\hat{\boldsymbol{U}}^{t}$\small\\
Make recommendations for the cold-start users
\caption{The \proposed framework}
\label{alg:framework}
\end{algorithm}
\setlength{\textfloatsep}{2.5pt}

\noindent \textbf{Discussion: the necessity of metric space for \cdr.} 
The fundamental motivation of \cdr is that users with similar tastes are located close to each other in the source-domain latent space, and they are likely to be located close in the target-domain latent space as well.
For this reason, the latent space for each domain should be able to capture user-user similarities as well as user-item interactions.
%However, the existing methods~\cite{EMCDR2017, dcdcsr2018, autoencoder_CDR_2019_AAAI} do not carefully consider this aspect;
%they learn the user-item interactions as the inner product of a user vector and an item vector, which makes the latent space violate the \textit{triangle inequality}~\cite{triangle_inequality_2012}.
%As pointed out in~\cite{CML, PME2018}, the user-user and item-item similarities are not accurately modeled in case that the triangle inequality is not guaranteed. 
%On the contrary, in the metric space that satisfies the triangle inequality, the user-user and item-item similarities are also captured with user-item interactions, because the users that share many interacted items (or the items that share many interacted users) get closer in the metric space \cite{CML}.
In the metric space that satisfies the triangle inequality, the user-user and item-item similarities are also captured with user-item interactions, because the users that share many interacted items (or the items that share many interacted users) get closer in the metric space \cite{CML}.
To this end, we model users and items in the metric space, which is also well compatible with the cross-domain mapping in the following subsections.

\subsection{Semi-Supervised Metric Space Mapping}
\label{subsec:mapping}
The second step of \proposed is to learn a mapping function that captures the relationship between the two metric spaces (i.e., target-domain metric space and source-domain metric space). 
To effectively learn the relationship even with a small number of overlapping users, we employ the idea of semi-supervised learning.
In general, semi-supervised learning \cite{semi_intro, SSL_ICML2008} aims at improving the overall performance of a supervised task when there are a small amount of labeled data and a large amount of unlabeled data.
The underlying concept of the semi-supervised learning is based on the local-consistency assumption, which means data samples with high similarity are likely to have the same label. 
This assumption aligns with the fundamental motivation of CDR.

We formulate the training of cross-domain mapping function as a semi-supervised task.
%We consider learning the mapping function as a supervised task.
We regard the overlapping users as the labeled data, because we have the ground-truths about the target-domain locations where their source-domain latent vectors should be transferred by the mapping function.
%Specifically, we regard their source-domain latent vectors as input data and target-domain latent vectors as ground-truths.
Without loss of generality, we can regard source-domain items that do not have ground-truths in the target-domain metric space as unlabeled data.
% we aim to improve the quality of latent space mapping by using rich unlabeled data based on its contexts (CF information) to the labeled data.

\vspace{2pt}
\noindent \textbf{Supervised Loss.}
The supervised loss uses the overlapping users as the labeled data.
The mapping function takes the user latent vectors in the source-domain as its inputs and the user latent vectors in the target-domain as the desired outputs.
The loss function can be described by
\begin{equation}
\label{eq:suploss}
    \begin{aligned}
    \mathcal { L } _ { S } &=  \sum _ { i \in \mathcal {O U} } d \left( f _ { \theta } \left( \mathbf { u }^s _ { i }\right) , \mathbf { u }^t _ { i } \right)_{,}
\end{aligned}
\end{equation}

\noindent
where $f _ { \theta } (\cdot)$ is the cross-domain mapping function, parameterized by $\theta$.
Note that the supervised loss tunes the location of each source-domain user vector transferred by the mapping function close to its ground-truth location in the target-domain metric space.
% MLP 내용은 실험 섹션에 넣자,..

\vspace{2pt}
\noindent \textbf{Unsupervised Loss.}
We design an effective unsupervised loss to involve the source-domain items into the training of the mapping function.
Although the ground-truth locations of the source-domain items do not exist in the target-domain metric space, the mapping function can further learn the inter-domain relationship so that it transfers CF information observed in the source-domain (i.e., user-item interactions) to the target-domain metric space. 
Concretely, we transfer the latent vectors of the source-domain items to the target-domain metric space through the mapping function, then adjust the transferred locations according to whether it has interacted with the overlapping users or not.
Based on this idea, we define the following unsupervised loss.
\begin{equation}
\label{eq:unsuploss}
\begin{aligned}
    \mathcal { L } _ {U} &=  \sum _ { i \in \mathcal{O U} } \sum _ { j \in \text{\neighborofuseri} } \sum _ { k \notin \text{\neighborofuseri} } \left[ m + d \left(f _ { \theta } (\mathbf { v }^s _ { j } ), \mathbf { u }^t _ {i} \right) - d \left( f _ { \theta } ( \mathbf { v }^s _ { k } ) , \mathbf { u }^t _ { i }\right) \right] _ { +, }
\end{aligned}
\end{equation}

\noindent
where $f _ { \theta } (\mathbf { v }^s _ { j } )$ is the transferred location of source-domain item $j$, $[x]_{+} = \max(x,0)$ is the standard hinge loss, and $m$ is the margin size.
This loss ensures that the distance of an observed user-item pair is smaller than that of an unobserved pair by a margin of $m$ in the target-domain metric space.
In other words, each overlapping user pulls (or pushes) its interacted (or non-interacted) source-domain items in the target-domain metric space.
The locations of the transferred item vectors are adjusted by the unsupervised loss, and the changes are propagated to their nearby users. 
That is, the transferred locations of cold-start users who have interacted with the items in the source-domain are also adjusted in the target-domain metric space.
% adjust 표현 괜찮은가?
% cold-start users로 전파되는 부분에 대한 설명 보충 필요

\vspace{2pt}
\noindent \textbf{The complete Loss function.}
The complete loss function for metric space mapping can be described as
\label{eq:completeloss}
\begin{equation}
\begin{aligned}
    & \hspace{10mm} \min _ { \theta} \mathcal { L } _ { S} + \lambda \cdot \mathcal { L } _ { U }\\
    & s.t.\hspace{3mm}||f_ { \theta}(\mathbf{u}_{*})||^2 \leq 1 \text{ and } ||f_ { \theta}(\mathbf{v}_{*})||^2 \leq 1.
\end{aligned}
\end{equation}

% 로스 argument로 theta를 넣는게 어떨지..?
\noindent
$\lambda$ is the weight hyperparameter that controls the importance of the unsupervised loss, and $\theta$ denotes the parameters of the mapping function.
%, which are weight matrices and biases.
The unit-sphere constraint is also enforced in the same way with Section~\ref{subsec:modeling}.

% implementation으로
%As our focus is to verify the benefit of the semi-supervised approach, we do not use advanced negative sample techniques \cite{negativesample2016, negativesamepling2}. For each observed user-item pair, we randomly sample one negative item that the user did not interact with.

\noindent \textbf{Discussion: the effect of the semi-supervised loss.} 
In case that the mapping function is trained by the supervised loss, the locations of users and items transferred by the mapping function are easily confined near to the overlapping users.
%The proposed semi-supervised loss is designed to alleviate this problem.
Figure~\ref{fig:method} illustrates how the semi-supervised mapping approach alleviates this problem.
In our complete loss function, the supervised loss (Eq.~\eqref{eq:suploss}) learns the labeled data as anchor points, and the unsupervised loss (Eq.~\eqref{eq:unsuploss}) makes the unlabeled data spread over the target-domain metric space according to their relative similarities to the anchors.
Our metric spaces correctly encode the similarity among entities (i.e., user and item), so the unlabeled source-domain items also can be involved in the training of the mapping function based on their similarity to the overlapping users.
As a result, the transferred locations of cold-start users are no longer biased to the overlapping users and get closer to the points that represent their preferences accurately.
% Note that this semi-supervised mapping is only valid for metric spaces, because both the losses learns the distances among users and items in the space.

\subsection{Multi-hop Neighborhood Inference}
\label{subsec:inference}
%Although just transferring source-domain user latent vector and then finding top-$N$ items (Section~\ref{subsec:emcdr}) also work well in \proposed, this process does not fully exploit the benefits by the metric learning and semi-supervised learning (we will discuss this in following discuss section). To this end, we propose a novel technique that infers latent vectors of the cold-start users by using a newly defined user latent vector. 
% , which has been shown to be effective for recommendation \cite{CDAE, neighborhood22016}. 
% mapping때 interaction을 반영한 바와 같이, inference 시에도 각 유저의 interaction을 반영한다. 
The final step of \proposed is to recommend target-domain items to cold-start users.
We propose an inference technique that accurately infers the latent vectors of the cold-start users by fully utilizing their multi-hop neighborhood\footnote{We use the term ``neighbors'' to represent the set of each user's interacted items and the set of each item's interacted users, rather than the nearest entities in a space.} information (i.e., a set of items interacted with a user, and a set of users interacted with an item)~\cite{CDAE, neighborhood22016}.
We first compute new vectors of the cold-start users in the source-domain metric space by repeatedly aggregating their neighbors, then transfer the vectors to the target-domain metric space by using the mapping function.

The $h$-th aggregated latent vectors of a user $i$ and an item $j$ in the source-domain metric space can be represented as
\begin{align}
     \mathbf {v}^{s,h} _ { j } &= \frac{1}{|\text{\neighborofitemj}|+1}  \bigg( \mathbf {v}^ { s,h-1}_ { j }  +  \sum_{i\in \text{\neighborofitemj}}\mathbf {u}^{s,h-1}_{i} \bigg), \\
    \mathbf{u}^{s,h} _ { i } &= \frac{1}{|\text{\neighborofuseri}|+1}  \bigg(\mathbf {u}^ { s,h-1}_ { i }  +  \sum_{j\in \text{\neighborofuseri}}\mathbf {v}^{s,h-1}_{j }\bigg).
\end{align}

\noindent
We set the initial vectors (in case of $h=0$) to the learned user and item vectors; $\mathbf {v} _ { j } ^ { s,0 } = \mathbf {v}^s _ { j }, \mathbf {u} _ {i } ^ { s,0 } = \mathbf {u}^s _ {i }$.
In this way, each final $H$-th aggregated user vector encompasses the information of both the user and its $H$-hop neighbors.
Finally, \proposed infers the latent vector of a cold-start user $i$ by
%using the aggregated user vector and the mapping function. 
%For example, given a cold-start user $i$, \proposed infer its latent vector in the target-domain metric space as follows:
\begin{equation}
    \hat { \mathbf { u } } _ { i } ^ { t } = f_ { \theta } ( \mathbf { u } _ { i } ^ { s,H } ),
\end{equation}
\noindent
and recommend the top-$N$ items, which are located nearest to the latent vector in the target-domain metric space, to the user.

\noindent \textbf{Discussion: the effect of the multi-hop neighborhood inference.}
% naive? straightforward? simple?
The naive inference of the cold-start users' preferences, which transfers their source-domain latent vectors to the target-domain by the trained mapping function, has a limited performance.
This is because their interactions in the source-domain are only considered implicitly (i.e., captured in their source-domain latent vectors).
To improve the accuracy of the inference, our proposed inference technique predicts the locations of the cold-start users by explicitly making use of their interactions (i.e., neighbors).
Their neighborhood information in the source-domain is helpful for the accurate inference, because our mapping function is trained to capture user-item interactions observed in the source-domain by the semi-supervised mapping approach.

%So, we try to adjust the locations of the cold-start users by using their neighborhood information.
%Note that the CF information (user-item interactions) in the source-domain is reflected in the mapping function through the semi-supervised approach.
%By aggregating the neighborhood information, we can adjust the position of the cold-start users considering both their information and their CF information.
%The semi-supervised approach adjusts the location of the cold-start users based on their relative similarities to the overlapping users.
%When the number of overlapping users is severely limited, it can be still challenging to elaborately adjust the locations of the cold-start users based on 
%Note that the CF information (user-item interactions) in the source-domain is reflected in the mapping function through the semi-supervised approach.
%By aggregating the neighborhood information, we can adjust the position of the cold-start users considering both their information and their CF information.




==> chapters/sscdr/sections/050experiments.tex <==
We conduct extensive experiments to evaluate our \proposed framework.
We first show the superior performance of \proposed over the state-of-the-art methods (Section~\ref{subsec:mainresult}), and analyze the effectiveness of each component in \proposed framework in the target-domain metric space (Section~\ref{subsec:targetmetric}).


\subsection{Experimental Setup}

\label{subsec:setting}
\begin{table}[h]
\centering
\setlength\tabcolsep{3.2pt}
  \renewcommand{\arraystretch}{0.80}
  \caption{Statistics of the cross-domain scenarios (Inter. denotes interactions and Overlap. denotes overlapping users)}
  \label{tbl:dataset}
  \begin{tabular}{ccccccc}
    \toprule
    && $\#$Users & $\#$Items & $\#$Inter.& Density & $\#${\small Overlap.} \\
    \midrule
    \multirow{2}{*}{Scenario 1} & Book  & 4,291 & 18,984 & 171,206 & 0.21\% & \multirow{2}{*}{1,823} \\
          & Video & 17,690 & 48,376 & 883,226 & 0.10\% &\\       
    \midrule
    \multirow{2}{*}{Scenario 2} & Music & 8,783 & 35,672 & 427,112 & 0.14\% & \multirow{2}{*}{1,306}  \\
          & Book  & 4,090 & 18,920 & 168,317 & 0.22\% & \\  
    \midrule
    \multirow{2}{*}{Scenario 3} & Video & 17,902 & 48,402 & 886,247 & 0.10\% & \multirow{2}{*}{2,029} \\
          & Game  & 3,680 & 12,416 & 104,465 & 0.23\% & \\    
    \bottomrule
\end{tabular}
\end{table}
%\vspace{-10pt}

\noindent
\textbf{Dataset.} We use the Amazon dataset.
Then, we define three \cdr scenarios as \textit{Scenario 1}: Book $\rightarrow$ Video, \textit{Scenario 2}: Music $\rightarrow$ Book, and \textit{Scenario 3}: Video $\rightarrow$ Game.
For each scenario, we filter out the overlapping users whose number of interacted items is fewer than 10, and also filter out non-overlapping users and items with fewer than 20 interactions ~\cite{hu2013personalized, NeuMF, CML, autoencoder_CDR_2019_AAAI, BPR}.
The details of our \cdr scenarios are summarized in Table~\ref{tbl:dataset}.%\footnote{We preprocess the data after grouping two datasets as a pair, so the statistic of a single domain can vary in different scenarios.} %Our preprocessing script and the datasets used for experiments will be released.}

\vspace{2pt}
\noindent
\textbf{Experimental Setup.}
% We randomly split the total overlapping users as 50\% for test (i.e., ground-truths for cold-start users) and 50\% for training.
% 공유 유저의 50% 를 랜덤하게 선택하여, 타겟 도메인에서 정보를 지운다. 이 지워진 유저들이 cold-start 유저이다.
% ground-truth 는 latent space 상에서 쓰니까 다른 표현
For each scenario, we randomly select 50\% of the total overlapping users and remove their information in the target-domain in order to utilize them as cold-start users for calculating the recommendation accuracy (i.e., test users).
To investigate the performance changes of \cdr methods with respect to the number of overlapping users, we restrict the number of the overlapping users similarly to the real-world distribution as presented in Section~\ref{sec:analysis}.
For each scenario, we build four training sets by randomly including only a certain fraction $\phi\in\{5\%, 10\%, 50\%, 100\%\}$ of the overlapping users who do not belong to the test users.
% all the overlapping users not included in each training dataset are also removed from the target-domain.

%all the overlapping users not included in each training dataset are also removed from the target-domain.
%We set the fractions to , denoted by $\phi$.
%Specifically, for dataset 1, we randomly select 912 users as cold-start users and 45, 90, 456 and 912 users as overlapping users for each fraction. 
%For dataset 2, we randomly select 488 users as cold-start users and 24, 48, 244 and 488 users as overlapping users for each fraction. 
%Finally, for dataset 3, we randomly select 1015 users as cold-start users and 50, 101, 507 and 1015 users as overlapping users for each fraction. 
\vspace{2pt}
\noindent
\textbf{Evaluation Protocols.} We follow the \textit{leave-one-out} evaluation protocol widely used in the Top-$N$ recommendation task~\cite{NeuMF, negativesample2016, conet2018, transCF}.
For each test user, we leave out a single interacted items for testing, and use the rest for training.
In our experiments, we leave out an additional interacted item for the validation.
To address the time-consuming issue of ranking all the items, we randomly sample 999 items among the items that have not interacted with the user (i.e., negative items), then evaluate how well each method can rank the test item higher than these negative items. 
We repeat this process of sampling a test/validation item and negative items five times and report the average results.
As we focus on the top-$N$ recommendation task based on implicit feedback, we evaluate the performance of each method by using the three ranking metrics: 
hit ratio (HR), normalized discounted cumulative gain (NDCG), and mean reciprocal rank (MRR). 
The HR H@$N$ simply measures whether the test item is present in the top-$N$ list:
\begin{equation*}
\text{H} @ N = \frac { 1 } { | \mathcal { U }_{test} | } \sum _ { i \in \mathcal { U} _{test} } \delta \left( p _ { i } \leq \text { top } N \right),    
\end{equation*}
where $\mathcal { U }_{test}$ is the set of the test users, $p_i$ is the hit position of the test item for the user $i$, and $\delta ( \cdot )$ is the indicator function. 
The NDCG N@$N$ and the MRR M@$N$ are position-aware ranking metrics that assign higher scores to the hits at upper ranks:
\begin{equation*}
\text{N} @ N = \frac { 1 } { | \mathcal { U } _{test} | } \sum _ { i \in \mathcal { U }_{test} } \frac { \log 2 } { \log \left( p _ { i } + 1 \right) }\text{, M} @ N = \frac { 1 } { | \mathcal { U }_{test} | } \sum _ { i \in \mathcal { U } _{test} } \frac { 1 } { p _ { i } }    
\end{equation*}

\vspace{2pt}
\noindent
\textbf{Baselines.} We categorize our baseline methods into three groups according to their approaches.
A method in the first group performs \textit{non-personalized} recommendations (i.e., a non-\cf method).
\begin{itemize}[leftmargin=*]
  \item \textbf{\itempop}: A simple method which makes a ranked list of all items in the target-domain by the number of their interactions (i.e., popularity). 
  This method provides benchmark performances of the non-personalized recommendation.
\end{itemize}

\noindent
The methods in the second group consider all domains as a single domain for \cdr~ \cite{hu2013personalized,CBMF2015}. 
%A traditional approach of dealing with cross-domain information is treating the cross-domain information as a single domain \cite{hu2013personalized}.
We construct a unified matrix in a collective manner so that it takes all users and items as its rows and columns, respectively. 
Then, we apply the state-of-the-art \cf methods designed for a single domain.
\begin{itemize}[leftmargin=*]
  \item \textbf{BPR~\cite{BPR}:} Bayesian personalized ranking method for implicit feedback datasets. 
  %It learns the user and the item latent factors by using matrix factorization and pairwise ranking loss. 
  It assumes that the items interacted with a user are more preferred than the items not interacted yet, and learns the pairwise ranking loss for latent vector modeling.
  The loss optimizes the order of scores defined by the inner product of user and item latent vectors. 
  
  \item \textbf{CML~\cite{CML}:} The state-of-the-art \cf method for implicit feedback datasets based on a metric learning approach. 
  It learns a joint metric space where users and items are embedded, and their distance is considered inversely proportional to the strength of the user's preference on the item. 
\end{itemize}

\noindent
The third group includes the state-of-the-art \cdr methods for cold-start users.
\begin{itemize}[leftmargin=*]
  \item \textbf{\cbmf~\cite{CBMF2015}:} Clustering-based matrix factorization for top-$N$ recommendation to cold-start users. 
  %with cross-domain information.
  Based on matrix factorization (\mf), it learns and utilizes latent vectors at the two-levels:  1) latent vectors of each user and item, 2) latent vectors of each user-cluster and item-cluster.
  %It additionally factorizes a cross-domain cluster-based coarse matrix to capture the shared interests among user and item clusters, when predicting the preferences of users on tiems.
  %By factorizing the coarse matrix, the preferences of users on items are computed at a cluster level to generate cross-domain recommendations.
  % to be polished
  
  \item \textbf{\emcdrbpr~\cite{EMCDR2017}:} Our main competitor which is the state-of-the-art \cdr framework for cold-start users.
  It learns a cross-domain mapping function after latent vector modeling by \bpr.\footnote{In case of a rating prediction task, probabilistic matrix factorization (\pmf) is used instead of \bpr in~\cite{EMCDR2017}, but we focus on top-$N$ ranking task in this paper.} 
  %As we focus on recommendations for implicit feedback, we choose \bpr which is a ranking-optimized method.
\end{itemize}

\noindent
Finally, we build three variants of \proposed by excluding 1) the semi-supervised loss and 2) the inference technique to validate the effectiveness of each proposed component.
%All of them use \cml in order to learn the latent factors of users and items in a metric space. 
%Note that \emcdrbpr and all the proposed methods have the same mapping network configuration.
\begin{itemize}[leftmargin=*]
  \item \textbf{\emcdrcml:} An ablation of \proposed. It neither uses the semi-supervised approach nor the inference technique. Unlike the previous \emcdr that uses \bpr for latent vector modeling, it applies \cml to take advantages of the metric space.
  \item \textbf{\proposednoinf} and \textbf{\proposedinf:} The proposed framework which trains a cross-domain mapping function based on the semi-supervised loss. \proposednoinf straightforwardly infers the cold-start users by the mapping function (i.e., uses the naive inference), whereas \proposedinf adopts the multi-hop neighborhood inference technique.
\end{itemize}

Note that there are several \cdr methods designed to recommend items only to the users who already have interacted items in the target-domain~\cite{dcdcsr2018,conet2018,CDRimprove2018,CDRforsparsityreduction}; 
they are not included in our baselines because they cannot provide recommendations to cold-start users.
In addition, there exist the \cdr methods that make use of side information such as demographic profiles of users (e.g. age, gender, and profession)~\cite{bayesian2018},  review texts~\cite{hu2018mtnet, autoencoder_CDR_2019_AAAI}, and item contents (e.g. plot and title of movie)~\cite{autoencoder_CDR_2019_AAAI, bayesian2018};
they are also not included in our baselines as they require such side information for \cdr. 

\vspace{3pt}
\noindent
\textbf{Implementation Details.} 
% 1) implem. details
We implement our framework and all the baselines using Tensorflow~\cite{abadi2016tensorflow} for efficient computations on GPU, and use the Adam optimizer~\cite{kingma2014adam} to train all the methods.
For the cross-domain mapping functions of \emcdrbpr, \emcdrcml, \proposednoinf and \proposed, we employ Multi-layer perceptron (MLP) which is mainly used in \cdr methods~\cite{EMCDR2017,dcdcsr2018,autoencoder_CDR_2019_AAAI}, and apply the same network configuration as suggested in~\cite{EMCDR2017}.
Their hidden layers have the shape of $[K \rightarrow 2 \times K \rightarrow K]$, and the $tanh$ is used as the activation function.

% 2) hyperparemeter tuning
For each scenario and method, the hyperparameters are tuned by grid searches using the validation set:
the initial learning rate for the Adam optimizer in $\{$0.1, 0.03 ,0.01, 0.003, 0.001, 0.0003, 0.0001$\}$, the dimension size of the latent vector in $\{$10, 30, 50, 100$\}$, the model regularizer (for \bpr and \cbmf) in $\{$0.01, 0.005, 0.001, 0.0005, 0.0001$\}$, the margin size (for CML-based methods) in $\{$0.5, 1.0, 1.5$\}$, the weight parameter (for \cbmf) in $\{$0.2, 0.4, 0.6, 0.8, 1.0$\}$ and the number of clusters for users and items (for \cbmf) is set to 100 which is provided by~\cite{CBMF2015}.
% \footnote{We empirically found that the performances are hardly affected by this hyper-parameter.}
%For EMCDR and the proposed methods, latent space embeddings of each domain are saved when the validation accuracy is the best. 
The hyperparameters for \proposednoinf and \proposedinf are tuned in the range of $\lambda\in\{$0.25, 0.5 ,0.75, 1.0$\}$ and $H\in\{$1,2,3,4$\}$. 
%\vspace{-8pt}


\subsection{Comparing Different Approaches}
\label{subsec:mainresult}

\begin{sidewaystable}
  \renewcommand{\arraystretch}{0.7}
%  \setlength\tabcolsep{7pt}
  \small
  \caption{Recommendation performances. Best results are in bold face. 
  \textit{Imp.sup} denotes the improvement of \proposed over \emcdrcml.
  We conduct the paired t-test with 0.05 level on H@10 and all \textit{Imp.best} are statistically significant.}
  \label{tbl:SOTA1}
%  \begin{tabular}{ccr|C{1.5cm}C{1.1cm}C{1.1cm}C{1cm}C{1.6cm}C{1.2cm} C{1.5cm}C{1.1cm}}
  \begin{tabular}{cZ|Z|ZZZZZ|ZZZ|ZZ}
    \toprule 
     & $\phi$ &  Metrics  &  \itempop  &  \bpr  &  \cml  &  \cbmf  & \emcdrbpr &  \emcdrcml  &  \proposednoinf  &  \proposedinf &  \textit{Imp.best} & \textit{Imp.sup} \\
\bottomrule
\multirow{24}{*}{\rotatebox[origin=c]{90}{Scenario 1 \quad\quad\quad\quad\quad}} & \multirow{6}{*}{5$\%$} &H@10 & 0.1267 & 0.1412 & 0.1434 & 0.1425 & 0.1994 & 0.2068 & 0.2285 & \textbf{0.2354} & 18.05$\%$ & 13.83$\%$\\
 &  &  H@20 & 0.2029 & 0.2220 & 0.2226 & 0.2141 & 0.2959 & 0.2979 & 0.3238 & \textbf{0.3313} & 11.96$\%$ & 11.21$\%$\\
 &  &  N@10 & 0.0646 & 0.0710 & 0.0737 & 0.0768 & 0.1079 & 0.1126 & 0.1247 & \textbf{0.1273} & 17.98$\%$ & 13.06$\%$\\
 &  &  N@20 & 0.0836 & 0.0930 & 0.0949 & 0.0946 & 0.1304 & 0.1343 & 0.1435 & \textbf{0.1531} & 17.41$\%$ & 14.00$\%$\\
 &  &  M@10 & 0.0459 & 0.0501 & 0.0527 & 0.0571 & 0.0801 & 0.0838 & 0.0932 & \textbf{0.0949} & 18.48$\%$ & 13.25$\%$\\
 &  &  M@20 & 0.0510 & 0.0576 & 0.0599 & 0.0617 & 0.0843 & 0.0888 & 0.0931 & \textbf{0.1033} & 22.54$\%$ & 16.33$\%$\\

\cmidrule{2-13}
& \multirow{6}*{10$\%$} &H@10 & 0.1267 & 0.1614 & 0.1636 & 0.1679 & 0.2178 & 0.2184 & 0.2329 & \textbf{0.2362} & 8.45$\%$ & 8.15$\%$\\
 &  &  H@20 & 0.2029 & 0.2481 & 0.2562 & 0.2505 & 0.3181 & 0.3144 & 0.3311 & \textbf{0.3341} & 5.03$\%$ & 6.27$\%$\\
 &  &  N@10 & 0.0646 & 0.0821 & 0.0822 & 0.0882 & 0.1169 & 0.1199 & 0.1265 & \textbf{0.1286} & 10.01$\%$ & 7.26$\%$\\
 &  &  N@20 & 0.0836 & 0.1012 & 0.1022 & 0.1071 & 0.1415 & 0.1435 & 0.1515 & \textbf{0.1529} & 8.06$\%$ & 6.55$\%$\\
 &  &  M@10 & 0.0459 & 0.0578 & 0.0593 & 0.0640 & 0.0862 & 0.0897 & 0.0943 & \textbf{0.0968} & 12.30$\%$ & 7.92$\%$\\
 &  &  M@20 & 0.0510 & 0.0610 & 0.0624 & 0.0673 & 0.0921 & 0.0953 & 0.1023 & \textbf{0.1027} & 11.51$\%$ & 7.76$\%$\\


\cmidrule{2-13}
 & \multirow{6}*{50$\%$} &H@10 & 0.1267 & 0.2015 & 0.2053 & 0.2083 & 0.2351 & 0.2345 & 0.2498 & \textbf{0.2536} & 7.87$\%$ & 8.14$\%$\\
 &  &  H@20 & 0.2029 & 0.2959 & 0.3032 & 0.2913 & 0.3390 & 0.3313 & 0.3526 & \textbf{0.3550} & 4.72$\%$ & 7.15$\%$\\
 &  &  N@10 & 0.0646 & 0.1104 & 0.1112 & 0.1110 & 0.1285 & 0.1315 & 0.1393 & \textbf{0.1404} & 9.26$\%$ & 6.77$\%$\\
 &  &  N@20 & 0.0836 & 0.1298 & 0.1308 & 0.1322 & 0.1570 & 0.1548 & 0.1626 & \textbf{0.1655} & 5.41$\%$ & 6.91$\%$\\
 &  &  M@10 & 0.0459 & 0.0828 & 0.0827 & 0.0815 & 0.0960 & 0.1003 & 0.1057 & \textbf{0.1064} & 10.83$\%$ & 6.08$\%$\\
 &  &  M@20 & 0.0510 & 0.0841 & 0.0832 & 0.0879 & 0.1059 & 0.1048 & 0.1096 & \textbf{0.1130} & 6.70$\%$ & 7.82$\%$\\

\cmidrule{2-13}
& \multirow{6}*{100$\%$} &H@10 & 0.1267 & 0.2158 & 0.2228 & 0.2239 & 0.2413 & 0.2417 & 0.2549 & \textbf{0.2562} & 6.17$\%$ & 6.00$\%$\\
 &  &  H@20 & 0.2029 & 0.3102 & 0.3170 & 0.3181 & 0.3445 & 0.3410 & 0.3543 & \textbf{0.3559} & 3.31$\%$ & 4.37$\%$\\
 &  &  N@10 & 0.0646 & 0.1171 & 0.1198 & 0.1203 & 0.1341 & 0.1373 & 0.1410 & \textbf{0.1451} & 8.20$\%$ & 5.68$\%$\\
 &  &  N@20 & 0.0836 & 0.1403 & 0.1419 & 0.1428 & 0.1575 & 0.1602 & 0.1664 & \textbf{0.1668} & 5.90$\%$ & 4.12$\%$\\
 &  &  M@10 & 0.0459 & 0.0872 & 0.0887 & 0.0890 & 0.1015 & 0.1049 & 0.1064 & \textbf{0.1115} & 9.85$\%$ & 6.29$\%$\\
 &  &  M@20 & 0.0510 & 0.0932 & 0.0929 & 0.0942 & 0.1052 & 0.1089 & 0.1135 & \textbf{0.1143} & 8.65$\%$ & 4.96$\%$\\
\bottomrule
  \end{tabular}
\end{sidewaystable}




\begin{sidewaystable}
  \renewcommand{\arraystretch}{0.7}
%  \setlength\tabcolsep{7pt}
  \small
  \caption{Recommendation performances. Best results are in bold face. 
  \textit{Imp.sup} denotes the improvement of \proposed over \emcdrcml.
  We conduct the paired t-test with 0.05 level on H@10 and all \textit{Imp.best} are statistically significant.}
  \label{tbl:SOTA2}
%  \begin{tabular}{ccr|C{1.5cm}C{1.1cm}C{1.1cm}C{1cm}C{1.6cm}C{1.2cm} C{1.5cm}C{1.1cm}}
  \begin{tabular}{cZ|Z|ZZZZZ|ZZZ|ZZ}
    \toprule 
     & $\phi$ &  Metrics  &  \itempop  &  \bpr  &  \cml  &  \cbmf  & \emcdrbpr &  \emcdrcml  &  \proposednoinf  &  \proposedinf &  \textit{Imp.best} & \textit{Imp.sup} \\
\bottomrule

\multirow{24}{*}{\rotatebox[origin=c]{90}{Scenario 2 \quad\quad\quad\quad}} & \multirow{6}*{5$\%$} &H@10 & 0.0988 & 0.0830 & 0.0918 & 0.0881 & 0.0834 & 0.0901 & 0.0976 & \textbf{0.1143} & 15.69$\%$ & 26.86$\%$\\
 &  &  H@20 & 0.1434 & 0.1295 & 0.1389 & 0.1246 & 0.1359 & 0.1409 & 0.1492 & \textbf{0.1656} & 15.48$\%$ & 17.53$\%$\\
 &  &  N@10 & 0.0557 & 0.0432 & 0.0451 & 0.0463 & 0.0434 & 0.0466 & 0.0482 & \textbf{0.0580} & 4.13$\%$ & 24.46$\%$\\
 &  &  N@20 & 0.0669 & 0.0546 & 0.0560 & 0.0557 & 0.0544 & 0.0572 & 0.0634 & \textbf{0.0697} & 4.19$\%$ & 21.85$\%$\\
 &  &  M@10 & 0.0409 & 0.0311 & 0.0310 & 0.0337 & 0.0314 & 0.0336 & 0.0334 & \textbf{0.0410} & 0.24$\%$ & 22.02$\%$\\
 &  &  M@20 & \textbf{0.0439} & 0.0331 & 0.0333 & 0.0366 & 0.0339 & 0.0345 & 0.0400 & 0.0434 & -1.14$\%$ & 25.80$\%$\\


\cmidrule{2-13}
 & \multirow{6}*{10$\%$} &H@10 & 0.0988 & 0.0914 & 0.0947 & 0.0934 & 0.0916 & 0.0967 & 0.1066 & \textbf{0.1152} & 16.60$\%$ & 19.13$\%$\\
 &  &  H@20 & 0.1434 & 0.1381 & 0.1422 & 0.1467 & 0.1418 & 0.1562 & 0.1651 & \textbf{0.1770} & 20.65$\%$ & 13.32$\%$\\
 &  &  N@10 & 0.0557 & 0.0456 & 0.0449 & 0.0475 & 0.0466 & 0.0505 & 0.0554 & \textbf{0.0596} & 7.00$\%$ & 18.02$\%$\\
 &  &  N@20 & 0.0669 & 0.0579 & 0.0584 & 0.0584 & 0.0596 & 0.0650 & 0.0681 & \textbf{0.0728} & 8.82$\%$ & 12.00$\%$\\
 &  &  M@10 & 0.0409 & 0.0323 & 0.0302 & 0.0336 & 0.0330 & 0.0366 & 0.0389 & \textbf{0.0428} & 4.65$\%$ & 16.94$\%$\\
 &  &  M@20 & 0.0439 & 0.0347 & 0.0356 & 0.0345 & 0.0362 & 0.0401 & 0.0417 & \textbf{0.0449} & 2.28$\%$ & 11.97$\%$\\


\cmidrule{2-13}
 & \multirow{6}*{50$\%$} &H@10 & 0.0988 & 0.1230 & 0.1259 & 0.1238 & 0.1236 & 0.1262 & 0.1365 & \textbf{0.1389} & 10.33$\%$ & 10.06$\%$\\
 &  &  H@20 & 0.1434 & 0.1918 & 0.1951 & 0.1906 & 0.1911 & 0.1938 & 0.2041 & \textbf{0.2070} & 6.10$\%$ & 6.81$\%$\\
 &  &  N@10 & 0.0557 & 0.0603 & 0.0613 & 0.0619 & 0.0642 & 0.0646 & 0.0682 & \textbf{0.0699} & 8.88$\%$ & 8.14$\%$\\
 &  &  N@20 & 0.0669 & 0.0783 & 0.0798 & 0.0763 & 0.0790 & 0.0804 & 0.0859 & \textbf{0.0862} & 8.02$\%$ & 7.19$\%$\\
 &  &  M@10 & 0.0409 & 0.0416 & 0.0418 & 0.0433 & 0.0463 & 0.0467 & 0.0478 & \textbf{0.0492} & 6.26$\%$ & 5.26$\%$\\
 &  &  M@20 & 0.0439 & 0.0474 & 0.0481 & 0.0466 & 0.0477 & 0.0496 & 0.0526 & \textbf{0.0531} & 10.40$\%$ & 7.14$\%$\\

\cmidrule{2-13}
& \multirow{6}*{100$\%$} &H@10 & 0.0988 & 0.1283 & 0.1320 & 0.1291 & 0.1320 & 0.1336 & 0.1372 & \textbf{0.1426} & 8.03$\%$ & 6.74$\%$\\
 &  &  H@20 & 0.1434 & 0.1975 & 0.2061 & 0.1996 & 0.1967 & 0.2037 & 0.2135 & \textbf{0.2184} & 5.97$\%$ & 7.22$\%$\\
 &  &  N@10 & 0.0557 & 0.0631 & 0.0665 & 0.0652 & 0.0658 & 0.0680 & 0.0693 & \textbf{0.0701} & 5.41$\%$ & 3.09$\%$\\
 &  &  N@20 & 0.0669 & 0.0849 & 0.0872 & 0.0855 & 0.0851 & 0.0879 & 0.0905 & \textbf{0.0909} & 4.24$\%$ & 3.41$\%$\\
 &  &  M@10 & 0.0409 & 0.0436 & 0.0468 & 0.0465 & 0.0478 & 0.0488 & 0.0494 & \textbf{0.0494} & 3.35$\%$ & 1.23$\%$\\
 &  &  M@20 & 0.0439 & 0.0534 & 0.0545 & 0.0546 & 0.0542 & 0.0552 & 0.0559 & \textbf{0.0565} & 3.48$\%$ & 2.36$\%$\\
\bottomrule
  \end{tabular}
\end{sidewaystable}


\begin{sidewaystable}
  \renewcommand{\arraystretch}{0.7}
%  \setlength\tabcolsep{7pt}
  \small
  \caption{Recommendation performances. Best results are in bold face. 
  \textit{Imp.sup} denotes the improvement of \proposed over \emcdrcml.
  We conduct the paired t-test with 0.05 level on H@10 and all \textit{Imp.best} are statistically significant.}
  \label{tbl:SOTA3}
%  \begin{tabular}{ccr|C{1.5cm}C{1.1cm}C{1.1cm}C{1cm}C{1.6cm}C{1.2cm} C{1.5cm}C{1.1cm}}
  \begin{tabular}{cZ|Z|ZZZZZ|ZZZ|ZZ}
    \toprule 
     & $\phi$ &  Metrics  &  \itempop  &  \bpr  &  \cml  &  \cbmf  & \emcdrbpr &  \emcdrcml  &  \proposednoinf  &  \proposedinf &  \textit{Imp.best} & \textit{Imp.sup} \\
\bottomrule

\multirow{24}{*}{\rotatebox[origin=c]{90}{Scenario 3 \quad\quad\quad\quad}} & \multirow{6}*{5$\%$} &H@10 & 0.0935 & 0.0830 & 0.0866 & 0.0876 & 0.0835 & 0.1024 & 0.1091 & \textbf{0.1179} & 26.10$\%$ & 15.14$\%$\\
 &  &  H@20 & 0.1540 & 0.1371 & 0.1391 & 0.1440 & 0.1367 & 0.1653 & 0.1712 & \textbf{0.1817} & 17.99$\%$ & 9.92$\%$\\
 &  &  N@10 & 0.0462 & 0.0398 & 0.0448 & 0.0418 & 0.0422 & 0.0532 & 0.0568 & \textbf{0.0597} & 29.22$\%$ & 12.22$\%$\\
 &  &  N@20 & 0.0613 & 0.0537 & 0.0572 & 0.0554 & 0.0576 & 0.0698 & 0.0723 & \textbf{0.0759} & 23.82$\%$ & 8.74$\%$\\
 &  &  M@10 & 0.0321 & 0.0270 & 0.0322 & 0.0354 & 0.0298 & 0.0385 & 0.0411 & \textbf{0.0430} & 21.47$\%$ & 11.69$\%$\\
 &  &  M@20 & 0.0362 & 0.0309 & 0.0347 & 0.0401 & 0.0350 & 0.0437 & 0.0452 & \textbf{0.0473} & 17.96$\%$ & 8.24$\%$\\

\cmidrule{2-13}
& \multirow{6}*{10$\%$} &H@10 & 0.0935 & 0.1065 & 0.1073 & 0.1105 & 0.1055 & 0.1177 & 0.1217 & \textbf{0.1286} & 16.38$\%$ & 9.26$\%$\\
 &  &  H@20 & 0.1540 & 0.1700 & 0.1744 & 0.1807 & 0.1639 & 0.1913 & 0.1963 & \textbf{0.1996} & 10.46$\%$ & 4.34$\%$\\
 &  &  N@10 & 0.0462 & 0.0509 & 0.0509 & 0.0527 & 0.0512 & 0.0611 & 0.0629 & \textbf{0.0663} & 25.81$\%$ & 8.51$\%$\\
 &  &  N@20 & 0.0613 & 0.0679 & 0.0720 & 0.0701 & 0.0686 & 0.0803 & 0.0817 & \textbf{0.0817} & 13.47$\%$ & 1.74$\%$\\
 &  &  M@10 & 0.0321 & 0.0343 & 0.0391 & 0.0354 & 0.0369 & 0.0440 & 0.0453 & \textbf{0.0476} & 21.74$\%$ & 8.18$\%$\\
 &  &  M@20 & 0.0362 & 0.0399 & 0.0439 & 0.0401 & 0.0424 & 0.0500 & 0.0504 & \textbf{0.0526} & 19.82$\%$ & 5.20$\%$\\

\cmidrule{2-13}
 & \multirow{6}*{50$\%$} &H@10 & 0.0935 & 0.1272 & 0.1292 & 0.1302 & 0.1345 & 0.1358 & 0.1404 & \textbf{0.1426} & 6.02$\%$ & 5.01$\%$\\
 &  &  H@20 & 0.1540 & 0.2039 & 0.2022 & 0.2028 & 0.2065 & 0.2093 & 0.2162 & \textbf{0.2199} & 6.49$\%$ & 5.06$\%$\\
 &  &  N@10 & 0.0462 & 0.0648 & 0.0672 & 0.0660 & 0.0706 & 0.0715 & 0.0724 & \textbf{0.0742} & 5.10$\%$ & 3.78$\%$\\
 &  &  N@20 & 0.0613 & 0.0845 & 0.0846 & 0.0837 & 0.0906 & 0.0879 & 0.0912 & \textbf{0.0923} & 1.88$\%$ & 5.01$\%$\\
 &  &  M@10 & 0.0321 & 0.0461 & 0.0487 & 0.0467 & 0.0505 & 0.0513 & 0.0520 & \textbf{0.0539} & 6.73$\%$ & 5.07$\%$\\
 &  &  M@20 & 0.0362 & 0.0516 & 0.0525 & 0.0511 & 0.0551 & 0.0546 & 0.0569 & \textbf{0.0578} & 4.90$\%$ & 5.86$\%$\\

\cmidrule{2-13}
 & \multirow{6}*{100$\%$} &H@10 & 0.0935 & 0.1353 & 0.1355 & 0.1385 & 0.1366 & 0.1406 & 0.1477 & \textbf{0.1481} & 6.93$\%$ & 5.33$\%$\\
 &  &  H@20 & 0.1540 & 0.2097 & 0.2172 & 0.2142 & 0.2136 & 0.2164 & 0.2239 & \textbf{0.2252} & 3.68$\%$ & 4.07$\%$\\
 &  &  N@10 & 0.0462 & 0.0683 & 0.0682 & 0.0694 & 0.0722 & 0.0740 & 0.0764 & \textbf{0.0766} & 6.09$\%$ & 3.51$\%$\\
 &  &  N@20 & 0.0613 & 0.0862 & 0.0907 & 0.0880 & 0.0901 & 0.0924 & 0.0951 & \textbf{0.0965} & 6.39$\%$ & 4.44$\%$\\
 &  &  M@10 & 0.0321 & 0.0482 & 0.0480 & 0.0488 & 0.0527 & 0.0538 & 0.0551 & \textbf{0.0552} & 4.74$\%$ & 2.60$\%$\\
 &  &  M@20 & 0.0362 & 0.0524 & 0.0562 & 0.0534 & 0.0566 & 0.0583 & 0.0598 & \textbf{0.0615} & 8.66$\%$ & 5.49$\%$\\

\bottomrule
  \end{tabular}
\end{sidewaystable}







We quantitatively evaluate the recommendation performance of \proposed and other methods in terms of three ranking metrics.
Table \ref{tbl:SOTA1}, Table \ref{tbl:SOTA2}, and Table \ref{tbl:SOTA3} show the results on three scenarios with four different $\phi$ values, which are the fractions of the overlapping users.
In summary, for all scenarios and $\phi$, \proposed achieves the best performance among all the baselines, and specifically, it shows the significant improvement (min: 6\%, max: 41\%, avg: 17\%) in terms of H@10 compared to the state-of-the-art method (i.e., \emcdrbpr).
We analyze the above results with various perspectives.

\vspace{1pt}
\noindent \textbf{The impact of the number of overlapping users.}
We observe that the performances of the existing methods are severely limited by the number of overlapping users.
Their performances drastically drop as the number of overlapping users decreases, and they even perform worse than the non-personalized recommendation method (i.e. \itempop). % personalized recommendation?
Specifically, in case of Scenario 2 with $\phi=5\%$ and $10\%$, every competitor shows worse performances than \itempop.
Likewise, in Scenario 3 with $\phi=5\%$, all the competitors except \emcdrcml are worse than \itempop.
In these settings, leveraging the knowledge obtained from another domain is no longer beneficial for the existing methods.
However, in the same settings, \proposedinf outperforms \itempop by up to 26.10\% (for H@10 in Scenario 3).
These results show that the proposed framework is capable of effectively exploiting the cross-domain knowledge even in the case that there are only a few overlapping users, and successfully overcomes the limitation of the existing methods.

\vspace{1pt}
\noindent \textbf{The effectiveness of the metric space.}
We observe that \emcdrcml outperforms \emcdrbpr, and CML outperforms BPR in general.
This tendency is consistent with the previous work~\cite{CML}, which verified the benefits of learning a metric space where the triangle inequality is satisfied.
This also emphasizes that the latent space should be able to correctly capture user-user similarity for cross-domain recommendation, as described in Section~\ref{subsec:modeling}.
% Also, in our experiment, the proposed semi-supervised latent space mapping and $k$-hop neighborhood inference have no positive effect when the latent spaces are learned by MF-based methods.

\vspace{1pt}
\noindent \textbf{The effectiveness of the semi-supervised mapping.}
We observe that \proposednoinf significantly outperforms \emcdrcml by up to 10.49$\%$ (for H@10 in Scenario 1 with $\phi=5\%$).
Notably, \proposednoinf recommends more accurately than \emcdrcml that uses double the number of overlapping users (for H@10 in Scenario 1 and Scenario 2 with $\phi=5\%$ (vs. 10$\%$) and 50$\%$ (vs. 100$\%$)). 
As \proposednoinf and \emcdrcml have the same mapping network configuration, their performance gap results from the proposed semi-supervised metric space mapping.
This results indicate that our semi-supervised approach achieves much better generalization compared to the supervised approach.

\vspace{1pt}
\noindent \textbf{The effectiveness of the multi-hop neighborhood inference.}
The superior performance of \proposedinf over \proposednoinf confirms that the proposed inference technique can infer more accurate latent vectors of the cold-start users than the naive inference, by effectively integrating their neighborhood information.

\begin{figure*}[th]
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[height=2.9cm]{chapters/sscdr/images/EMCDR.png}
    \caption{\small\emcdrcml}
\end{subfigure}%
    \hfill\hfill
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[height=2.9cm]{chapters/sscdr/images/SSCDR_no_INF.png}
    \caption{\small\proposednoinf}
\end{subfigure} 
    \hfill%
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[height=2.9cm]{chapters/sscdr/images/SSCDR.png}
    \caption{\small\proposed ($H=2$)}
\end{subfigure} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[height=2.9cm]{chapters/sscdr/images/SSCDR_INF_4.png}
    \caption{\small\proposedinf ($H=4$)}
\end{subfigure}%
    \hfill\hfill
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[height=2.9cm]{chapters/sscdr/images/Total.png}
    \caption{\small\emcdrcml and \proposedinf ($H=2$)}
\end{subfigure} 
    \hfill%
\begin{subfigure}[t]{0.33\linewidth}
    \includegraphics[height=2.9cm]{chapters/sscdr/images/Total_u3.png}
    \caption{\small \emcdrcml and \proposedinf ($H=2$)}
\end{subfigure} 
\caption{t-SNE visualization of transferred user latent vectors in target-domain metric space}
%\vspace{-10pt}
\label{fig:TSNE}
\end{figure*}


\subsection{Target-Domain Metric Space Analysis}
\label{subsec:targetmetric}
We conduct both qualitative and quantitative analyses on target-domain metric space to further investigate why \proposed outperforms the state-of-the-art methods. 
For the qualitative analysis, we visualize the target-domain metric space by using t-distributed Stochastic Neighbor Embedding (t-SNE)\footnote{We employ the default setting of the t-SNE provided by Scikit-learn~\cite{pedregosa2011scikit}.}~\cite{tsne2008} to observe how the inferred locations of the cold-start users\footnote{The test users have no ground-truths in the target-domain metric space. Thus, in this experiment, we use the overlapping users of each scenario with $\phi=100\%$, by splitting them into 5\% for training the mapping function and the other 95\% for testing with their ground-truths (i.e., cold-start users).} are affected by the semi-supervised mapping and the multi-hop neighborhood inference.
For the quantitative analysis, we measure the actual distances between the inferred latent vectors and their ground-truths.

Figure~\ref{fig:TSNE} shows the target-domain metric space in case of Scenario~1.
Red points represent the inferred latent vectors by \emcdrcml, and green points represent the inferred latent vectors by \proposed. 
Blue points represent ground-truth vectors of the cold-start users.
%\footnote{The cold-start users for testing have no ground-truths in the target-domain metric space. Thus, in this experiment, we consider the overlapping users which are not used for training the cross-domain mapping function (i.e., the remaining 95\%) as cold-start users, and plot their vectors.}
Black points and translucent circles represent the overlapping users and their surrounding areas, respectively.

\noindent
\textbf{How does the semi-supervised loss affect the mapping function? (\emcdrcml vs. \proposednoinf)}
%We observe that the semi-supervised approach helps the mapping function not to be biased to the overlapping users and to achieve improved generalization.
In Figure~\ref{fig:TSNE}(a), the red points are mostly located within the translucent circles, showing that the mapping function is severely biased to the overlapping users.
On the contrary, in Figure~\ref{fig:TSNE}(b), the green points are not confined to the circles but scattered over the target-domain metric space.
That is, the semi-supervised approach helps the mapping function not to be biased to the overlapping users and to achieve better generalization than the supervised approach.

\noindent
\textbf{How does the multi-hop neighborhood inference affect the transfer between two domains? (\proposednoinf vs. \proposedinf)}
%We observe that the proposed inference technique contributes to accurately infer the latent vectors of the cold-start users. 
The green points in Figure~\ref{fig:TSNE}(c) more overlap with the ground-truth blue points, compared to Figure~\ref{fig:TSNE}(b).
This implies that the inference technique effectively integrates neighborhood information to accurately predict the locations of the cold-start users.
We can also observe the effect of different degrees of the aggregation (i.e., $H$) in Figure~\ref{fig:TSNE}(c) and (d).

\noindent
\textbf{Does \proposed indeed infer more accurate latent vectors of the cold-start users? (\emcdrcml vs. \proposed)}
In Figure~\ref{fig:TSNE}(e), we visualize the latent vectors inferred by \emcdrcml (red points) and \proposed (green points) at once.
As shown in Figure~\ref{fig:TSNE}(a) and (c), the red points are clustered near the overlapping users (black points), whereas the green points are well mixed with the ground-truth points (blue points).
Figure~\ref{fig:TSNE}(f) provides the further analysis on ten users; the points with the same number represent the the same user. 
We confirm that \proposed indeed transfers the cold-start users to more accurate locations than \emcdrcml, and based on the inferred vectors, it can provide better recommendations.

==> chapters/sscdr/sections/060related.tex <==
We briefly survey the literature on \cdr methods developed for two different target user groups: 1) target-domain users and 2) cold-start users.
%Recent \cdr methods can be largely divided into two major categories according to their purpose.

\noindent
\textbf{\cdr methods for target-domain users.}
Most \cdr methods aim to improve the recommendation accuracy for the users in the target-domain~\cite{dcdcsr2018, conet2018, CDRimprove2018,CDRforsparsityreduction}. 
These methods integrate the knowledge acquired from the source-domain and the target-domain to improve the quality of recommendations in a collective manner. 
DCDCSR~\cite{dcdcsr2018} first computes combined user latent vectors by a convex combination of the latent vectors respectively obtained from the source-domain and target-domain, weighted by each user's rating sparsity. 
Then it learns a mapping function that captures the relationship from the target-domain latent vectors to the combined latent vectors. 
CoNet~\cite{conet2018} transfers and combines the knowledge by using cross-connections between feed-forward neural networks, which are used for a base network for each domain.
MINDTL~\cite{CDRimprove2018} combines the CF information of the target-domain with the rating patterns extracted from a cluster-level rating matrix in the source-domain.
Although all these methods are effective in improving the overall recommendation accuracy for target-domain users, they cannot make recommendations for cold-start users who do not interacted with any items.
%Thus, we do not compare them with \proposed in our experiments.

\vspace{3pt}
\noindent
\textbf{\cdr methods for cold-start users.}
Several approaches have been proposed to recommend target-domain items to cold-start users~\cite{EMCDR2017, CBMF2015, autoencoder_CDR_2019_AAAI, hu2018mtnet}.
CBMF~\cite{CBMF2015} first factorizes a cluster-based cross-domain coarse matrix to learn the shared preferences within user and item clusters. 
%By factorizing the coarse matrix, the preferences of users on items are computed at a cluster level.
Then it performs cross-domain recommendations by linearly combining the user-item interactions at the cluster-level and the user-level.
EMCDR~\cite{EMCDR2017} proposes a general \cdr framework. 
It learns a mapping function between the latent spaces of the source-domain and target-domain, by formulating the learning procedure as a supervised regression problem.
On the other hand, due to the technical difficulties of the recommendation to cold-start users in the absence of CF information, most studies have focused on side information for user and item modeling~\cite{bayesian2018, hu2018mtnet, autoencoder_CDR_2019_AAAI}. 
MVDNN~\cite{MVDNN2015} and GCBAN~\cite{bayesian2018} exploit users' demographic information (e.g. age, gender, and profession) or items' contextual information (e.g. genre of music, singer's name and publisher).
RC-DFM~\cite{autoencoder_CDR_2019_AAAI} employs Additional Stacked Denoising Autoencoder (aSDAE)~\cite{aSDAE2017} to fuse such side information with CF information, then learns a mapping function by supervised regression.
Our work is distinguished from the above methods in that we do not use any auxiliary data sources and also learn the cross-domain mapping based on a semi-supervised approach which is effective even in the case that only a small number of labeled data is available.

% 이전 relatied work
\begin{comment}
\noindent
\textbf{Metric Learning}
Metric learning aims at learning a distance metric that preserves the similarity among the training data. 
It has been actively studied in various domains such as natural language processing \cite{metric_nlp_2006} and computer vision \cite{metric_vision_2013}. 
Metric learning approach recently have been adopted in collaborative filtering to solve the limitation of matrix factorization \cite{CML, metric2_2010}. 
CML \cite{CML} is a state-of-the-art recommendation framework for implicit feedback.
CML projects users and items into a joint Euclidean space where user-item relationships and user-user/item-item similarity are computed based on the Euclidean distance.

\noindent
\textbf{Semi-supervised Learning}
Semi-supervised learning aims at increasing the performance of the supervised task by using a small amount of labeled data in conjunction with a large amount of unlabeled data. 
It has been successfully adopted in many areas such as computer vision \cite{semi_vision1,semi_vision2,semi_vision3} and network embedding \cite{ seminetwork1_2018, seminetwork2_2016}. 
A core assumption in many semi-supervised methods is the local-consistency assumption: data samples with high similarity are likely to have the same label. 
It is often used to regularize the classifiers trained from labeled samples.
In this work, we apply semi-supervised approach on cross-domain recommendation task.
Based on the similarity between unlabeled data and labeled data in the source-domain, we add unsupervised loss to improve the generation performance of the mapping function that learns the relationship between the two domains. 
In this way, rich unlabeled entities are appropriately reflected into the training of the model.
\end{comment}


